Tri-criterion model for constructing low-carbon mutual fund portfolios: a preference-based multi-objective genetic algorithm approach

Sustainable finance, which integrates environmental, social and governance (ESG) criteria on financial decisions rests on the fact that money should be used for good purposes. Thus, the financial sector is also expected to play a more important role to decarbonise the global economy. To align financial flows with a pathway towards a low-carbon economy, investors should be able to integrate in their financial decisions additional criteria beyond return and risk to manage climate risk. We propose a tri-criterion portfolio selection model to extend the classical Markowitz mean-variance approach in order to include investors preferences on the portfolio carbon risk exposure as an additional criterion. To approximate the 3D Pareto front we apply an efficient multi-objective genetic algorithm called ev-MOGA which is based on the concept of e-dominance. Furthermore, we introduce an a posteriori approach to incorporate the investor's preferences into the solution process regarding their sustainability preferences measured by the carbon risk exposure and his/her loss-adverse attitude. We test the performance of the proposed algorithm in a cross section of European SRI open-end funds to assess the extent to which climate related risk could be embedded in the portfolio according to the investor's preferences.

==> Low_Carbon_parameters.tex <==
\renewcommand{\arraystretch}{1.0}
    \begin{tabular}{ll}
    \hline
    Parameter & Value\\
  \hline
    Size of the main population  & $Nind_P=10^4$\\
    Size of the auxiliary population   & $Nind_{GA}=500$ \\
    Maximum algorithm iterations  & $k_{max}=10^5$\\
    Probability of crossing/mutation  & $P_{m/c}=0.2$ \\
    Number of boxes &  500\\
	\hline
    \end{tabular}%
